Grouped star formation: converting sink particles to stars in hydrodynamical simulations

Modelling star formation and resolving individual stars in numerical simulations of molecular clouds and galaxies is highly challenging. Simulations on very small scales can be sufficiently well resolved to consistently follow the formation of individual stars, whilst on larger scales sinks that have masses sufficient to fully sample the IMF can be converted into realistic stellar populations. However, as yet, these methods do not work for intermediate scale resolutions whereby sinks are more massive compared to individual stars but do not fully sample the IMF. In this paper, we introduce the grouped star formation prescription, whereby sinks are first grouped according to their positions, velocities, and ages, then stars are formed by sampling the IMF using the mass of the groups. We test our grouped star formation method in simulations of various physical scales, from sub-parsec to kilo-parsec, and from static isolated clouds to colliding clouds. With suitable grouping parameters, this star formation prescription can form stars that follow the IMF and approximately mimic the original stellar distribution and velocity dispersion. Each group has properties that are consistent with a star-forming region. We show that our grouped star formation prescription is robust and can be adapted in simulations with varying physical scales and resolution. Such methods are likely to become more important as galactic or even cosmological scale simulations begin to probe sub-parsec scales.

==> tables_tex/tab_distance.tex <==
\begin{table}
    \centering
    \begin{tabular}{l|l|l|l|l}
    \hline \hline
    Model            & $P_{25\%}$ & $P_{50\%}$  &$P_{75\%}$ &$P_{90\%}$ \\
    \hline \hline 
    B12NoGrouping    & 0.0010 & 0.0028 & 0.0059 & 0.0129 \\
    B12Standard      & 0.0008 & 0.0025 & 0.0054 & 0.0132 \\
    B12Turbulent     & 0.0003 & 0.0008 & 0.0034 & 0.0086 \\
    B12AllGrouping   & 0.0019 & 0.0039 & 0.0077 & 0.0256 \\
    \hline 
    L20NoGrouping    & 0.006 & 0.019 & 0.065 & 0.208 \\
    L20Standard      & 0.008 & 0.031 & 0.096 & 0.264 \\
    L20Turbulent     & 0.010 & 0.034 & 0.120 & 0.365 \\
    L20AllGrouping   & 0.011 & 0.054 & 0.209 & 0.647 \\
    \hline \hline
    \end{tabular}
    \caption{The 25\%, 50\%, 75\%, and 90\% percentile of the distance of stars from their parent sink particles for the chosen models, in the units of pc. }
    \label{tab:distance_sink_star}
\end{table}
